Statistical Modeling of Airborne Virus Transmission Through Imperfectly Fitted Face Masks

The rapid emergence and the disastrous impact of the severe acute respiratory syndrome coronavirus 2 (SARS-CoV-2) pandemic on public health, societies, and economies around the world has created an urgent need for understanding the pathways critical for virus transmission. Airborne virus transmission by asymptomatic SARS-CoV-2-infected individuals is considered to be a major contributor to the spread of SARS-CoV-2 and social distancing and wearing of face masks in public have been implemented as countermeasures in many countries. However, a comprehensive risk assessment framework for the airborne transmission of SARS-CoV-2 incorporating realistic assumptions on the filtration of infectious aerosols (IAs) by face masks is not available yet. In particular, in most end-to-end models for airborne virus transmission, it is neglected that the stochastic spread of IAs through imperfectly fitted face masks depends on the dynamics of the breathing of the wearer. In this paper, we consider airborne virus transmission from an infected but asymptomatic person to a healthy person, both wearing imperfectly fitted face masks, in an indoor environment. By framing the end-to-end virus transmission as a Molecular Communications (MC) system, we obtain a statistical description of the number of IAs inhaled by the healthy person subject to the respective configurations of the face masks of both persons. We demonstrate that the exhalation and inhalation air flow dynamics have a significant impact on the stochastic filtering of IAs by the face masks. Furthermore, we show that the fit of the face mask of the infected person can highly impact the infection probability. We conclude that the proposed MC model may contribute a valuable assessment tool to fight the spread of SARS-CoV-2 as it encompasses the randomness of the transmission process and enables comprehensive risk analysis beyond statistical averages.

==> end-to-end_transmission.tex <==
Let the binary RV $S_j$ denote the event that IA $j$ is transmitted from the IP to the HP via airborne transmission, i.e., $S_j = 1$ if IA $j$ is transmitted and $S_j = 0$ otherwise.
According to the results presented in Sections~\ref{sec:transmitter}, \ref{sec:channel}, and \ref{sec:receiver}, we can write $S_j$ as
\begin{align}
    S_j = \Stx_j \Sch_j \Srx_j,
\end{align}
where we have adopted the convention that $\Sch_j = \Srx_j = 0$ if $\Stx_j = 0$ and $\Srx_j = 0$ if $\Sch_j = 0$.
Accordingly,
\begin{align}
    \Pr\lbrace S_j = 1 \rbrace &= \Pr\lbrace\Stx_j = 1, \Sch_j = 1, \Srx_j = 1 \rbrace = 1 - \Pr\lbrace S_j = 0 \rbrace \nonumber\\
    &= \Pr\lbrace\Stx_j = 1\rbrace \Pr\lbrace \Sch_j = 1 | \Stx_j = 1\rbrace \Pr\lbrace\Srx_j = 1 | \Stx_j = 1, \Sch_j = 1 \rbrace,
\end{align}
and the random number of inhaled IA by the HP, IIA, is given by
\begin{align}
    \textrm{IIA} = \sum_{j = 1}^{J} S_j.
\end{align}
Note that the $S_j$ are independent Bernoulli RVs, but they are not identically distributed due to the dependence of the exhalation and inhalation probability on the random exhalation and inhalation times of each IA, respectively.
Hence, the RV IIA does in general not follow the Binomial distribution.

